Memory-Based Dual Gaussian Processes for Sequential Learning

Sequential learning with Gaussian processes (GPs) is challenging when access to past data is limited, for example, in continual and active learning. In such cases, errors can accumulate over time due to inaccuracies in the posterior, hyperparameters, and inducing points, making accurate learning challenging. Here, we present a method to keep all such errors in check using the recently proposed dual sparse variational GP. Our method enables accurate inference for generic likelihoods and improves learning by actively building and updating a memory of past data. We demonstrate its effectiveness in several applications involving Bayesian optimization, active learning, and continual learning.

==> fig/split_mnist/split_mnist_acc_proposed.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
height=\figureheight,
tick align=outside,
tick pos=left,
width=\figurewidth,
y grid style={darkgray176},
ylabel={Accuracy},
ytick style={color=black}
]
\addplot [semithick, steelblue31119180, opacity=0.5]
table {%
0 0.0896481732070365
1.33333333333333 0.175913396481732
2.66666666666667 0.559878213802436
4 0.969553450608931
};
%\addlegendentry{Proposed}
\addplot [semithick, steelblue31119180, opacity=0.5, forget plot]
table {%
4 0.49766557150268
5.33333333333333 0.515995158222376
6.66666666666667 0.582569600553346
8 0.858205083866505
};
\addplot [semithick, steelblue31119180, opacity=0.5, forget plot]
table {%
8 0.588990607537748
9.33333333333333 0.889192723814053
10.6666666666667 0.887528236832719
12 0.887528236832719
};
\addplot [semithick, steelblue31119180, opacity=0.5, forget plot]
table {%
12 0.664028457092041
13.3333333333333 0.890618052467763
14.6666666666667 0.88377056469542
16 0.889195197865718
};
\addplot [semithick, steelblue31119180, opacity=0.5, forget plot]
table {%
16 0.714826453363805
17.3333333333333 0.779602913869447
18.6666666666667 0.875660619911441
20 0.881302671046993
};
\addplot [semithick, steelblue31119180, opacity=0.5, forget plot]
table {%
0 0.0977672530446549
1.33333333333333 0.205683355886333
2.66666666666667 0.278416779431664
4 0.983085250338295
};
\addplot [semithick, steelblue31119180, opacity=0.5, forget plot]
table {%
4 0.501642745979595
5.33333333333333 0.566660902645686
6.66666666666667 0.715891405844717
8 0.827943973716064
};
\addplot [semithick, steelblue31119180, opacity=0.5, forget plot]
table {%
8 0.571989061942694
9.33333333333333 0.886577101414814
10.6666666666667 0.866722149566044
12 0.865533230293663
};
\addplot [semithick, steelblue31119180, opacity=0.5, forget plot]
table {%
12 0.646776345042241
13.3333333333333 0.871765228990663
14.6666666666667 0.889284126278346
16 0.877100933748333
};
\addplot [semithick, steelblue31119180, opacity=0.5, forget plot]
table {%
16 0.704899300099986
17.3333333333333 0.770961291244108
18.6666666666667 0.885230681331238
20 0.890372803885159
};
\addplot [semithick, steelblue31119180, opacity=0.5, forget plot]
table {%
0 0.0933694181326116
1.33333333333333 0.229702300405954
2.66666666666667 0.551420838971583
4 0.974289580514208
};
\addplot [semithick, steelblue31119180, opacity=0.5, forget plot]
table {%
4 0.497492650873249
5.33333333333333 0.745114992218572
6.66666666666667 0.810133148884662
8 0.843852671623725
};
\addplot [semithick, steelblue31119180, opacity=0.5, forget plot]
table {%
8 0.57864700986803
9.33333333333333 0.864700986802996
10.6666666666667 0.856735227678041
12 0.851979550588515
};
\addplot [semithick, steelblue31119180, opacity=0.5, forget plot]
table {%
12 0.635660293463762
13.3333333333333 0.898532681191641
14.6666666666667 0.868385949310805
16 0.901111605157848
};
\addplot [semithick, steelblue31119180, opacity=0.5, forget plot]
table {%
16 0.723968004570776
17.3333333333333 0.799957148978717
18.6666666666667 0.875017854592201
20 0.877017568918726
};
\addplot [semithick, steelblue31119180, opacity=0.5, forget plot]
table {%
0 0.106901217861976
1.33333333333333 0.128890392422192
2.66666666666667 0.288227334235453
4 0.979025710419486
};
\addplot [semithick, steelblue31119180, opacity=0.5, forget plot]
table {%
4 0.500086460314716
5.33333333333333 0.605740964897112
6.66666666666667 0.605740964897112
8 0.83831921148193
};
\addplot [semithick, steelblue31119180, opacity=0.5, forget plot]
table {%
8 0.576863630959458
9.33333333333333 0.899298537629295
10.6666666666667 0.88170253239805
12 0.882891451670432
};
\addplot [semithick, steelblue31119180, opacity=0.5, forget plot]
table {%
12 0.659226322810138
13.3333333333333 0.894797687861272
14.6666666666667 0.900578034682081
16 0.890884837705647
};
\addplot [semithick, steelblue31119180, opacity=0.5, forget plot]
table {%
16 0.71489787173261
17.3333333333333 0.74053706613341
18.6666666666667 0.860234252249679
20 0.877446079131553
};
\addplot [semithick, steelblue31119180, opacity=0.5, forget plot]
table {%
0 0.0991204330175913
1.33333333333333 0.118064952638701
2.66666666666667 0.538565629228687
4 0.963125845737483
};
\addplot [semithick, steelblue31119180, opacity=0.5, forget plot]
table {%
4 0.49126750821373
5.33333333333333 0.511499221857168
6.66666666666667 0.642918900224797
8 0.812726958326128
};
\addplot [semithick, steelblue31119180, opacity=0.5, forget plot]
table {%
8 0.559148733800975
9.33333333333333 0.89323504934015
10.6666666666667 0.886577101414814
12 0.87659017952681
};
\addplot [semithick, steelblue31119180, opacity=0.5, forget plot]
table {%
12 0.654779902178746
13.3333333333333 0.87967985771454
14.6666666666667 0.889817696754113
16 0.884215206758559
};
\addplot [semithick, steelblue31119180, opacity=0.5, forget plot]
table {%
16 0.710041422653907
17.3333333333333 0.749464362233967
18.6666666666667 0.878660191401228
20 0.883159548635909
};

\end{axis}

\end{tikzpicture}

